Diffusion Tuning: Transferring Diffusion Models via Chain of Forgetting

Diffusion models have significantly advanced the field of generative modeling. However, training a diffusion model is computationally expensive, creating a pressing need to adapt off-the-shelf diffusion models for downstream generation tasks. Current fine-tuning methods focus on parameter-efficient transfer learning but overlook the fundamental transfer characteristics of diffusion models. In this paper, we investigate the transferability of diffusion models and observe a monotonous chain of forgetting trend of transferability along the reverse process. Based on this observation and novel theoretical insights, we present Diff-Tuning, a frustratingly simple transfer approach that leverages the chain of forgetting tendency. Diff-Tuning encourages the fine-tuned model to retain the pre-trained knowledge at the end of the denoising chain close to the generated data while discarding the other noise side. We conduct comprehensive experiments to evaluate Diff-Tuning, including the transfer of pre-trained Diffusion Transformer models to eight downstream generations and the adaptation of Stable Diffusion to five control conditions with ControlNet. Diff-Tuning achieves a 26% improvement over standard fine-tuning and enhances the convergence speed of ControlNet by 24%. Notably, parameter-efficient transfer learning techniques for diffusion models can also benefit from Diff-Tuning.

==> alg_diff-tuning.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}[H]
\small

\caption{Pseudo-code of Diff-Tuning}
\label{alg}
\begin{algorithmic}
\STATE \textbf{Input:} Downstream dataset $\mathcal{X}$, pre-trained model parameter $\theta_0$ \\
\STATE \textbf{Output:} Fine-tuned parameter $\theta$.
\STATE Collect pre-sampled data $\widehat{\mathcal{X}}^s$ for knowledge reconsolidation using $\theta_0$.
\STATE Initialize $\theta\gets\theta_0$.
\WHILE{not converged}
\STATE Sample a mini-batch $\widehat{X}^s=\left\{\widehat{\mathbf{x}}_0^{s,(1)},...,\widehat{\mathbf{x}}_0^{s,(B/2)}\right\}$ of size $B/2$ from $\widehat{\mathcal{X}}^s$.
\STATE Calculate mini-batch retention loss
$$
L_\text{retention}(\theta) \gets \sum\limits_{\widehat{\mathbf{x}}_0^{s}\in \widehat{X}^s}\mathbb{E}_{\bm{\epsilon},t\sim\mathrm{catecorial}(\xi(t))} \left[\left\|\bm{\epsilon} - f_\theta\left(\sqrt{\alpha_t}\mathbf{\hat{x}}^{s}_0+\sqrt{1-\alpha_t}\bm{\epsilon}, t\right)\right\|^2\right],
$$
$\quad$ with weighted sampling of $t$ and the simple loss form.
\STATE Sample a mini-batch $X=\left\{\mathbf{x}_0^{(1)},...,\mathbf{x}_0^{(B/2)}\right\}$ of size $B/2$ from $\mathcal{X}$.
\STATE Calculate mini-batch adaptation loss
$$
L_\text{adaptation}(\theta) \gets \sum\limits_{\mathbf{x}\in X}\mathbb{E}_{\bm{\epsilon},t\sim\mathrm{catecorial}(\psi(t))} \left[\left\|\bm{\epsilon} - f_\theta\left(\sqrt{\alpha_t}\mathbf{x}_0+\sqrt{1-\alpha_t}\bm{\epsilon}, t\right)\right\|^2\right],
$$
$\quad$ with weighted sampling of $t$ and the simple loss form.
\STATE Calculate $L(\theta)\gets L_\text{retention}(\theta)+L_\text{adaptation}(\theta)$.
\STATE Update $\theta$ according to $\nabla_\theta L(\theta)$.
\ENDWHILE
\RETURN $\theta$
\end{algorithmic}
\end{algorithm}

==> tab-control-apdx.tex <==

\begin{table}[ht]
\centering
\caption{Detailed setting of quantitative metrics for controlled generation tasks.}
\begin{small}
\begin{tabular}{@{}l|cccccc@{}}
\toprule
                    & Edge                    & Sketch                    & Depth             & Normal             & Seg. (COCO)           & Seg. (ADE20k)           \\ \midrule
Metric              & \multicolumn{2}{c}{SSIM w/ Blurring ($\uparrow$)} & \multicolumn{2}{c}{MSE ($\downarrow$)} & \multicolumn{2}{c}{Pixel Accuracy ($\uparrow$)} \\
Threshold           & 0.55                    & 0.75                      & 0.04              & 0.06               & 0.5                   & 0.4                     \\ \midrule
ControlNet          & 6.7k                    & 3.8k                      & 9.9k              & 10.3k              & 9.2k                  & 13.9k                   \\
ControlNet+Diff-Tuning & 5.3k                    & 3.2k                      & 8.8k              & 7.8k               & 6.3k                  & 8.3k                    \\ \bottomrule
\end{tabular}
\end{small}
\label{table: controlnet-detail}
\end{table}

==> tab-control.tex <==
\begin{table*}[ht]
	\centering
    \vspace{-5pt}
    \caption{Sudden convergence steps on controlling Stable Diffusion with 5 conditions.}
    \vspace{0.1cm}
	\setlength{\tabcolsep}{3.2pt}
	\scalebox{0.95}{\begin{tabular}{l|cccccc|c}
			\toprule
			Method & Sketch & Normal & Depth  & Edge & Seg. (COCO) & Seg. (ADE20k) &  Average  \\
            \midrule
			ControlNet~\citep{controlnet-zhang2023adding}                     & 3.8k & 10.3k & 9.9k & 6.7k & 9.2k & 13.9k & 9.0k \\
            \midrule
             ControlNet +\textbf{Diff-Tuning}              & \textbf{3.2k} & \textbf{7.8k} & \textbf{8.8k} & \textbf{5.3k} & \textbf{6.3k} & \textbf{8.3k} & \textbf{6.6k} \\
             Relative Promotion & 15.8\% & 24.3\% &  11.1\% &  20.9\% & 31.5\% &  40.3\% &  24.0\%
            \tabularnewline
			\bottomrule 
		\end{tabular}
 	}
        \normalsize

	\label{table: fine-tuning-controlnet-sudden}
	\vspace{-0.2cm}
\end{table*}

==> tab-downstream.tex <==



\begin{table*}[bh]
    \setlength{\abovecaptionskip}{-0.01cm}
    \setlength{\belowcaptionskip}{-0.1cm}
    \caption{Comparisons on 8 downstream tasks with pre-trained DiT-XL-2-256x256. Methods with "\dag" are reported from the original Table 1 of \cite{difffit-xie2023difffit}. Parameter-efficient methods are denoted by "*".}
    \vskip 0.1in
    \centering
    \setlength{\tabcolsep}{2.0pt}
    \scalebox{0.95}{\begin{tabular}{l|cccccccc|c}
    \toprule
    \diagbox{Method}{Dataset}&\makecell[c]{~Food~} & ~SUN~ & \makecell[c]{DF-20M}  & \makecell[c]{Caltech}  & \makecell[c]{CUB-Bird} & \makecell[c]{ArtBench} & \makecell[c]{~Oxford~ \\ Flowers} & \makecell[c]{~Standard~ \\ Cars} &  \makecell[c]{Average \\ FID} \\
    \midrule
    Full Fine-tuning                     & 10.68 & 11.01 & \underline{14.74} & 29.79 & 5.32 & 20.59 & 16.67 & 6.04 & 14.36  \\
    AdaptFormer$^{\dag*}$\citep{adaptformer-chen2022adaptformer}  & 11.93 & 10.68 & 19.01 & 34.17 & 7.00 & 35.04  & 21.36 & 10.45 & 18.70 \\
    BitFit$^{\dag*}$\citep{bitfit-zaken2021bitfit}                & 9.17 & \underline{9.11} & 17.78 & 34.21 & 8.81 & 24.53   & 20.31 & 10.64 & 16.82 \\
    VPT-Deep$^{\dag*}$\citep{vpt-jia2022visual}               & 18.47 & 14.54 & 32.89 & 42.78 & 17.29 & 40.74 & 25.59 & 22.12 & 26.80  \\
    LoRA$^{\dag*}$\citep{lora-hu2021lora}                 & 33.75 & 32.53 & 120.25 & 86.05 & 56.03 & 80.99 & 164.13 & 76.24 & 81.25 \\
    DiffFit$^{*}$\citep{difffit-xie2023difffit}              & \underline{7.80} & 10.36 & 15.24 & \underline{26.81} &\underline{4.98} & \underline{16.40} & \underline{14.02} & \underline{5.81} & \underline{12.81} \\
    \midrule
     \textbf{Diff-Tuning}              & \textbf{6.05} & \textbf{7.21} & \textbf{12.57} & \textbf{23.79} & \textbf{3.50} & \textbf{13.85} & \textbf{12.64} & \textbf{5.37} & \textbf{10.63} \\

    Relative Promotion & 43.4\% & 34.5\% & 14.7\% & 20.1\% & 34.2\% & 32.7\% & 24.2\% & 11.1\% & 26.0\% \\
    \bottomrule 
    \end{tabular}
    }
    \vspace{0.5cm}
    \label{table: fine-tuning-downstream-datasets}
    \vspace{-0.3cm}
\end{table*}


==> tab-hyper-parameter.tex <==

\begin{table}[h]
\centering
\caption{Hyperparameters of experiments.}
\label{table: hyperparameter}
\begin{tabular}{@{}l|cc@{}}
\toprule
                    & Class-conditional & Controlled            \\ \midrule
Backbone            & DiT               & Stable-diffusion v1.5 \\
Image Size          & 256               & 512                   \\
Batch Size          & 32                & 4                     \\
Learning Rate       & 1e-4              & 1e-5                  \\
Optimizer           & Adam              & Adam                  \\
Training Steps      & 24000             & 15000                 \\
Validation Interval & 24000             & 100                   \\
Sampling Steps      & 50                & 50                    \\
\bottomrule
\end{tabular}
\end{table}

